Metric-VLA: Closing the Loop Between 3D Object Pose and Action

Vision-language-action (VLA) policies learn diverse manipulation skills from large-scale, task-oriented datasets, yet often struggle with metric instructions such as "move the bottle 10 cm to the right". Following these commands requires tracking the object's motion and determining how much remains to reach the target, quantities that current VLAs typically leave implicit. We present Metric-VLA, which closes the loop directly between 3D object pose and action. A goal reasoner combines visual grounding with geometric composition to translate the instruction into a 3D object goal pose. Two continuous pose tokens provide the action expert with the current pose of the commanded object and its remaining residual to the goal. After each action chunk, a CAD-free tracker fuses visual tracks with gripper kinematics to update the object pose and goal residual. The consequence of acting becomes the next condition for planning. We evaluate metric instructions, spatial relations, and their compositions using the achieved object pose. For this, we introduce LIBERO-Pose and ROP to benchmark simulated and real robot actions. On LIBERO-Pose, Metric-VLA outperforms the strongest of seven learned baselines, raising overall success from 17.4% to 71.3%; on ROP, it improves over $\pi_{0.5}$ from 24.0% to 72.7%. Project page: https://colin-de.github.io/Metric-VLA/

==> figures/teaser/sq_fpart_overlay.tex <==
\draw[tdirstart] (0.476,0.432) -- (0.234,0.518);
\draw[tdirgoal] (0.513,0.449) -- (0.472,0.620);
\node[tlab] at (0.459,0.671) {forward};


==> figures/teaser/sq_pos_overlay.tex <==
\draw[tdim] (0.652,0.394) -- (0.338,0.396);
\node[tlab] at (0.496,0.327) {12.5\,cm};

